On the Manipulability of Voting Systems: Application to Multi-Carrier Networks

Today, Internet involves many actors who are making revenues on it (operators, companies, service providers,...). It is therefore important to be able to make fair decisions in this large-scale and highly competitive economical ecosystem. One of the main issues is to prevent actors from manipulating the natural outcome of the decision process. For that purpose, game theory is a natural framework. In that context, voting systems represent an interesting alternative that, to our knowledge, has not yet been considered. They allow competing entities to decide among different options. Strong theoretical results showed that all voting systems are susceptible to be manipulated by one single voter, except for some "degenerated" and non-acceptable cases. However, very little is known about how much a voting system is manipulable in practical scenarios. In this paper, we investigate empirically the use of voting systems for choosing end-to-end paths in multi-carrier networks, analyzing their manipulability and their economical efficiency. We show that one particular system, called \Single Transferable Vote (STV), is largely more resistant to manipulability than the natural system which tries to get the economical optimum. Moreover, STV manages to select paths close to the economical optimum, whether the participants try to cheat or not.

==> abstract.tex <==
%\thispagestyle{empty}

\begin{abstract}

Today, Internet involves many actors who are making revenues on it (operators, companies, service providers,...). It is therefore important to be able to make fair decisions in this large-scale and highly competitive economical ecosystem. One of the main issues is to prevent actors from manipulating the natural outcome of the decision process. For that purpose, game theory is a natural framework.

In that context, voting systems represent an interesting alternative that, to our knowledge, has not yet been considered. They allow competing entities to decide among different options. Strong theoretical results showed that all voting systems are susceptible to be manipulated by one single voter, except for some ``degenerated'' and non-acceptable cases. However, very little is known about how much a voting system is manipulable in practical scenarios. 

In this paper, we investigate empirically the use of voting systems for choosing end-to-end paths in multi-carrier networks, analyzing their manipulability and their economical efficiency.  
We show that one particular system, called \emph{Single Transferable Vote} (STV), is largely more resistant to manipulability than the natural system which tries to get the economical optimum. Moreover, STV manages to select paths close to the economical optimum, whether the participants try to cheat or not.
\end{abstract}

\begin{IEEEkeywords}
Voting systems, game theory, manipulability, multi-carrier networks.
\end{IEEEkeywords}



==> figures.tex <==
\label{sec:figures}


\begin{figure}
\centering
\includegraphics[width=0.90\textwidth]{Fig_IntercarrierNetworkExample.png}
\caption{Multi-carrier network model}
\label{fig_icn}
\vspace{-.5cm}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.90\textwidth]{Fig_Manipulability.png}
\caption{Manipulability of STV vs. Range Voting}
\label{fig_manip}
%\vspace{-.5cm}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.90\textwidth]{Fig_SincereEfficiency.png}
\caption{Efficiency of STV vs. Range Voting for sincere preferences}
\label{fig_eff_sincere}
%\vspace{-.5cm}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.90\textwidth]{Fig_ManipulatedEfficiency.png}
\caption{Efficiency of STV vs. Range Voting for manipulated preferences}
\label{fig_eff_manip}
%\vspace{-.5cm}
\end{figure}


==> manipulability.tex <==
\vspace{-.1cm}
\section{Manipulability of voting systems}
\label{sec:manipulability}
\vspace{-.1cm}

TO BE REMOVED with cleaning of other parts: remove ref. to §III...


